3DInAction: Understanding Human Actions in 3D Point Clouds

We propose a novel method for 3D point cloud action recognition. Understanding human actions in RGB videos has been widely studied in recent years, however, its 3D point cloud counterpart remains under-explored. This is mostly due to the inherent limitation of the point cloud data modality -- lack of structure, permutation invariance, and varying number of points -- which makes it difficult to learn a spatio-temporal representation. To address this limitation, we propose the 3DinAction pipeline that first estimates patches moving in time (t-patches) as a key building block, alongside a hierarchical architecture that learns an informative spatio-temporal representation. We show that our method achieves improved performance on existing datasets, including DFAUST and IKEA ASM. Code is publicly available at https://github.com/sitzikbs/3dincaction.

==> assets/figs/ASM_vis/asm_vis_fig.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/ASM_vis/TV_Bench_christian/000087_img.png}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/ASM_vis/TV_Bench_christian/000135_img.png}
    \end{subfigure}
        \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/ASM_vis/TV_Bench_christian/001934_img.png}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/ASM_vis/TV_Bench_christian/002133_img.png}
    \end{subfigure}

        \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={3cm 5cm 3cm 3cm}, clip]{assets/figs/ASM_vis/TV_Bench_christian/000087_pc.png}}{align leg}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={3cm 5cm 3cm 3cm}, clip]{assets/figs/ASM_vis/TV_Bench_christian/000135_pc.png}}{spin leg}
    \end{subfigure}
        \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={3cm 5cm 3cm 3cm}, clip]{assets/figs/ASM_vis/TV_Bench_christian/001934_pc.png}}{flip table}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={3cm 5cm 3cm 3cm}, clip]{assets/figs/ASM_vis/TV_Bench_christian/002133_pc.png}}{attach shelf}
    \end{subfigure}
    \caption{\textbf{IKEA ASM Dataset actions images and point clouds.} Visualizing the RGB image (top), 3D point cloud (middle), and action label (bottom) for the TV bench assembly.}
    \label{fig:IKEA_ASM_examles}
\end{figure*}

==> assets/figs/Ego_vis/ego_vis_fig.tex <==
\begin{figure*}
    \centering
    
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/spin_screwdriver_img.png}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/attach_side_panel_img.png}
    \end{subfigure}
        \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/slide_bottom_panel_img.png}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/spin_drawer_knob_img.png}
    \end{subfigure}

        \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={11cm 0cm 11cm 0cm}, clip]{assets/figs/Ego_vis/spin_screwdriver_pc.png}}{spin screwdriver}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={11cm 0cm 11cm 0cm}, clip]{assets/figs/Ego_vis/attach_side_panel_pc.png}}{attach side panel}
    \end{subfigure}
        \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={11cm 0cm 11cm 0cm}, clip]{assets/figs/Ego_vis/slide_bottom_panel_pc.png}}{slide bottom panel}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={11cm 0cm 11cm 0cm}, clip]{assets/figs/Ego_vis/spin_drawer_knob_pc.png}}{spin drawer knob}
    \end{subfigure}

    \medskip
    \hrulefill\par
    \vspace{10pt}

        \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/stool/use_drill_img.png}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/stool/attach_stool_side_img.png}
    \end{subfigure}
        \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/stool/flip_stool_img.png}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \includegraphics[width=.99\linewidth]{assets/figs/Ego_vis/stool/align_top_stool_step_img.png}
    \end{subfigure}

        \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={16cm 1cm 15cm 3cm}, clip]{assets/figs/Ego_vis/stool/use_drill_pc.png}}{use drill}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={12cm 0cm 12cm 0cm}, clip]{assets/figs/Ego_vis/stool/attach_stool_side_pc.png}}{attach stool side}
    \end{subfigure}
        \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={11cm 0cm 11cm 0cm}, clip]{assets/figs/Ego_vis/stool/flip_stool_pc.png}}{flip stool}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    \centering
        \stackunder[5pt]{\includegraphics[width=.99\linewidth, trim={11cm 0cm 11cm 0cm}, clip]{assets/figs/Ego_vis/stool/align_top_stool_step_pc.png}}{align top stool step}
    \end{subfigure}
    


    \caption{\textbf{IKEA Ego 3D Dataset actions.} Visualizing the RGB image (top), 3D point cloud (middle), and action label (bottom) for the drawer, stool and TV bench assemblies.}
    \label{fig:IKEA_Ego_examles}
\end{figure*}

==> assets/tables/NTU_results.tex <==
\begin{table}[]\scriptsize 
    \centering
    \setlength\tabcolsep{4pt}
    \begin{tabular}{l c c c c}
         \toprule
         \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{NTU60}} & \multicolumn{2}{c}{\textbf{NTU120}} \\
         \cmidrule(lr){2-3}\cmidrule(lr){4-5}
         & Subject & View & Subject & Setup \\
        \hline
         PointNet++ \cite{qi2017pointnet++} &80.1&85.1&72.1&79.4 \\
         3DV \cite{wang20203dv} &84.5&95.4&76.9&92.5 \\
         3DV-PointNet++ \cite{wang20203dv} &88.8&96.3&82.4&93.5 \\
         PSTNet \cite{fan2021pstnet} &90.5&96.5&87.0&93.8 \\
         P4Transformer \cite{fan2021p4transformer} &90.2&96.4&86.4&93.5 \\
         PST-Transformer \cite{fan2022psttransformer} &91.0&96.4&87.5&94.0 \\
         Ours &&&& \\
         \bottomrule
    \end{tabular}
    \caption{ \textbf{Action classification on NTU dataset.}}
    \label{tab:results:baseline:ntu}
\end{table}

==> assets/tables/action_segmentation_3D.tex <==
\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c}
         \toprule
            \multirow{2}{*}{\textbf{Method}} &  \multicolumn{2}{c}{\textbf{Frame acc.}}    \\
            & \textbf{top 1} & \textbf{top 3} & \textbf{macro} & \textbf{mAP}\\
            \hline
            I3D - RGB \cite{carreira2017quo} & 56.39 & 75.78 & 43.44 & 28.82\\
            \hline
            I3D - Depth - baseline & 34.35 & 60.87 & 24.87 & 14.82\\
            I3D - Depth - Watch TV - L2  & 27.37 & 55.38 & 21.28 & 17.02\\
            I3D - Depth - Watch TV - cos  & 45.6 & 70.25 & 33.25 & 24.24\\
            I3D - Depth - Watch TV - cos no logits replace  & 45.2 & 70.09 & 34.3 & 23.76\\
            \hline
            PN4D - per frame - no agg - no T & 10.07 & 28.78 & 10.2 & 4.68\\
            PN4D - per frame - no agg - w T & 15.77 & 36.7 & 13.53 & 5.1 \\
            PN4D + w agg - w T & 12.75 & 25.28 & 13.51 &5.63 \\
            PN4D + w agg - w T - w Watch TV tune all & 12.63 & 24.07 & 13.34 & 4.99\\
            PN4D + w agg - w T - w Watch TV tune  fc & 12.15 & 21.12 & 11.34 & 6.21 \\
            PN4D - per frame - no agg - w T  - w Watch TV & 8.76  & 22.44  & 11.02  & 4.74 \\
            \hline
            PN\textsuperscript{++}4D - per frame - baseline & 43.21  & 68.58  & 28.97  & 13.21 \\
            PN\textsuperscript{++}4D - agg SA1 & 47.04  & 69.41  & 29.98  & 12.53 \\
            % PN\textsuperscript{++}4D - agg SA2 &   &   &   &  \\
            PN\textsuperscript{++}4D - agg SA1 - watch TV & 45.49  & 71.02 &  20.71  & 15.1 \\
         \bottomrule
    \end{tabular}
    \caption{Action recognition baseline frame-wise accuracy, macro-recall, and mean average precision results.}
    \label{tab:results:baseline:action_segmentation_3D}
\end{table}


\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c}
         \toprule
            \multirow{2}{*}{\textbf{Method}} &  \multicolumn{2}{c}{\textbf{Frame acc.}}    \\
            & \textbf{top 1} & \textbf{top 3} & \textbf{macro} & \textbf{mAP}\\
            \hline
            I3D - RGB \cite{carreira2017quo} & 56.39 & 75.78 & 43.44 & 28.82\\
            I3D - Depth - baseline & 34.35 & 60.87 & 24.87 & 14.82\\
            \hline
            PN4D - per frame  & 12.83 & 32.61 & 12.12 & 4.16\\
            PN4D + temporal smoothing &   &   &   &  \\
            PN\textsuperscript{++}4D - per frame - baseline & 43.21  & 68.58  & 28.97  & 13.21 \\
            PN\textsuperscript{++}4D + temporal smoothing&   &   &   &  \\


            \hline
            Ours + Sinkhorn &   &   &   &  \\ 
            &   &   &   &  \\

         \bottomrule
    \end{tabular}
    \caption{Action recognition baseline frame-wise accuracy, macro-recall, and mean average precision results.}
    \label{tab:results:baseline:action_segmentation_3D_new}
\end{table}

==> assets/tables/action_segmentation_front_view.tex <==
\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c}
         \toprule
            \multirow{2}{*}{\textbf{Method}} &  \multicolumn{2}{c}{\textbf{Frame acc.}}    \\
            & \textbf{top 1} & \textbf{top 3} & \textbf{macro} & \textbf{mAP}\\
            \hline
            ResNet18 \cite{he2016deep} & 27.06 & 55.14 & 21.95 & 11.69\\
            ResNet50 \cite{he2016deep} &  30.38 & 56.1 & 20.03 & 9.47\\
            C3D \cite{tran2015learning} & 45.73 & 69.56  & 32.48 & 21.98\\
            P3D \cite{Qiu_2017_ICCV} & \textbf{60.4} & \textbf{81.07} & \textbf{45.21} & \textbf{29.86}\\
            % VGG19 & &  \\
            I3D \cite{carreira2017quo} & 57.58 & 76.72 & 39.03 & 28.77\\
         \bottomrule
    \end{tabular}
    \caption{Action recognition baseline frame-wise accuracy, macro-recall, and mean average precision results.}
    \label{tab:results:baseline:action_segmentation}
\end{table}


==> assets/tables/action_segmentation_modalities.tex <==
\begin{table}[]\scriptsize
\setlength\tabcolsep{3pt}
    \centering
    \begin{tabular}{l l c c c c}
         \toprule
            \multirow{2}{*}{\textbf{Data type}}& \multirow{2}{*}{\textbf{View}} &  \multicolumn{2}{c}{\textbf{Frame acc.}}    \\
               & & \textbf{top 1} & \textbf{top 3} & \textbf{macro} & \textbf{mAP}\\

            \hline
            \multirow{4}{*}{RGB}&top view   & 57.58 & 76.72 & 39.03 & 28.77\\ %dev3
            &front view & 60.75 & 79.3 & 42.67 & 32.73\\ %dev2
            &side view  & 52.16 & 72.21 & 36.59 & 26.76\\ %dev1
            &combined views & 63.09 & 80.54 & 45.23 & 32.37 \\
            \hline
            Human pose & HCN \cite{li2018co} & 39.15 & 65.37 & 28.18 & 22.32\\
            Human pose & ST-GCN \cite{yan2018spatial} &  43.4 & 66.29 & 26.54 & 18.56\\
            &combined RGB+pose & 64.25 & 80.58 & 46.33 & 33.08\\
            \hline
            Depth & top view  & 35.43 & 59.48 & 21.37 & 14.4\\
            \hline
            &combined all & 64.02 & 81.45 & 44.61 & 31.45\\

         \bottomrule
    \end{tabular}
    \caption{Action recognition frame-wise accuracy, macro-recall, and mean average precision results for multi-view/modal inputs.}
    \label{tab:results:baseline:action_segmentation_modalities}
\end{table}

==> assets/tables/corr_exp.tex <==
\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c c}
         \toprule
            \multirow{2}{*}{\textbf{Method}} &  \multicolumn{5}{c}{\textbf{Accuracy}} \\
            & clean & $\sigma$=1\% & $\sigma$=0.5\% & $\sigma$=0.25\% & $\sigma$=0.1\% \\
            \hline
            NN  & 82.28 & 39.59 & 60.73 & 74.17& 80.65\\
            Sinkhorn  & 94.47 & 46.6  & 71.15 & 85.71 & 92.88\\
            \hline
            Ours SSL & 89.64 & 33.4 & &&\\
            Ours clean old & 95.6  &  & &  & \\
            Ours clean 840 & 86.61  & 37.28 & 59.91 & 75.31 & 84.11\\
            Ours clean 1290 &  &  & & & \\
            Ours noisy old & 95.55 &  34.62 & &&\\
            Ours clean 1 & 94.4 & 35.59  & 58.77 & 76.97 &89.68\\
            Ours clean 2 & 93.26 &   &  &  &86.67\\
         \bottomrule
    \end{tabular}
    \caption{Correspondence accuracy on the DFAUST dataset \cite{}. Comparing baseline point matching methods to the proposed correspondence transformer. Details: 1024 points, random sampling}
    \label{tab:results:baseline:correspondance}
\end{table}

% 1 : dfaust_N1024ff1024_d1024h8_ttypenonelr0.0001bs8debug_ce
% 2 : dfaust_N1024ff1024_d1024h8_ttypenonelr0.0001bs32reg_cat_ce2

\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c c}
         \toprule
            \multirow{2}{*}{\textbf{Method}} &  \multicolumn{5}{c}{\textbf{Accuracy}} \\
            & clean & $\sigma$=0.1\% & $\sigma$=0.25\% & $\sigma$=0.5\% & $\sigma$=1\% \\
            \hline
            NN  & 96.25 & 96.14 & 95.53 & 91.75 & 62.43\\
            Sinkhorn  100 & 98.54 &  98.52 & 98.39 & 97.67 & 78.09\\
            Sinkhorn  10 & 97.53 & 97.5  & 97.29 & 96.13 & 73.67\\
            \hline
            Ours 1 & 97.80  & 97.5 & 95.61 & 86.17 & 53.9\\
            Ours 2 & 97.97 & 97.18 & 94.79 & 90.00 & 66.27\\
            Ours Set TRM & 99.51 & & 95.98 &  & 55.71\\
            Ours Set TRM +noise  & 99.37 & & 98.18 & 95.14 & 73.05\\
         \bottomrule
    \end{tabular}
    \caption{Correspondence accuracy on the DFAUST dataset \cite{}. Comparing baseline point matching methods to the proposed correspondence transformer. Details: 1024 points, fps\_each sampling}
    \label{tab:results:baseline:correspondance_fps}
\end{table}

% 1 dfaust_N1024ff1024_d1024h8_ttypenonelr0.0001bs32fps_l2/150, Note: kept improving 
% 2 dfaust_N1024ff1024_d1024h8_ttypenonelr0.0001bs32fps_l2_jitter0.01/250, Note: kept improving 
% Ours Set TRM +noise: dfaust_N1024ff1024_d1024h8_ttypeset_transformerlr0.0001bs8debug_set_transformer_ce2_jitter/000700.pt

==> assets/tables/dataset_comparison.tex <==
\begin{table}[]\scriptsize
\setlength\tabcolsep{3pt}
    \centering
    \begin{tabular}{l c c c c c c c c}
        \toprule
         \textbf{Dataset} &  \textbf{Year}  & \textbf{\#Frames}   & \textbf{\#cls}& \textbf{ Ego view}\\
         \hline
         % Drive\&Act \cite{drive_and_act_2019_iccv} & 2019 &12h &  30 & 9.6M & driving  \\
         MSR-Action 3D \cite{li2010msraction3d}& 2010  & 23K  & 20  & \xmark\\
         NTU RGB+D 60 \cite{shahroudy2016ntu} &  2016  & 4M   & 60  & \xmark \\
        DFAUST \cite{dfaust:CVPR:2017} &         2017  & 45K  & 14  & \xmark\\
         NTU RGB+D 120 \cite{liu2019ntu}&        2019  & 8M   & 120 &\xmark\\

         IKEA-ASM \cite{ikeaasm}&                2020  & 3M   & 33  & \xmark\\
         \hline
         Our IKEA Ego 3D &                       2023  & 493K & 56  & \cmark\\
          \bottomrule
    \end{tabular}
    \vspace{-0.5em}
    \caption{3D point cloud action recognition datasets.}
    \vspace{-0.5em}
    \label{tab:dataset_comp}
\end{table}

==> assets/tables/ikeaego_results.tex <==
\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c}
         \toprule
            \multirow{2}{*}{\textbf{Method}} &  \multicolumn{2}{c}{\textbf{Frame acc.}}    \\
            & \textbf{top 1} & \textbf{top 3} & \textbf{macro} &  \textbf{mAP}\\
            \hline
            I3D & 65.56 & 92.99 & 56.04 &  0.6670 \\
            \hline
            % PointNet \cite{qi2017pointnet} & 32.17 & 63.25 & 22.03 & 0.0745 \\
            % PoinNet + t-smoothing & 31.28 & 60.26 & 17.15 & 0.0765 \\
            % PointNet$^{++}$ \cite{qi2017pointnet++} & 41.03 & 77.65 & 28.55 & 0.0869 \\
            % PointNet$^{++}$ \cite{qi2017pointnet++} + t-smooth & 39.29 & 78.11 & 30.59 & 0.0961 \\
            % \hline
            % Ours & 34.18 & 71.47 & 24.96 & 0.0994 \\
            PointNet$^{++}$ \cite{qi2017pointnet++}  & 52.08 & 78.65 & 22.83 &  0.3795\\
            Set Transformer \cite{lee2019settransformer} & 42.04 & 70.57 & 16.13 & 0.2141 \\
            \hline
            PointNet$^{++}$ \cite{qi2017pointnet++} + TS &  &  &  &  \\
            Set Transformer \cite{lee2019settransformer} + TS & 44.80 & 73.30 & 21.39 & 0.2944 \\
            \hline
            Ours & &  &  &  \\
         \bottomrule
    \end{tabular}
    \caption{IKEA Ego 3D results.}
    \label{tab:results:baseline:ikeaego}
\end{table}

% \begin{table}[]\scriptsize
%     \centering
%     \begin{tabular}{l c c c c}
%          \toprule
%             \multirow{2}{*}{\textbf{Method}} &  \multicolumn{2}{c}{\textbf{Frame acc.}}    \\
%             & \textbf{top 1} & \textbf{top 3} & \textbf{macro} &  \textbf{mAP}\\
%             \hline
%             % PointNet \cite{qi2017pointnet} & 33.51 & 84.93 & 38.90 & 0.08607 \\
%             % PoinNet + t-smoothing  & 29.88 & 90.15 & 31.79 & 0.07974 \\
%             % PointNet$^{++}$ \cite{qi2017pointnet++} & 50.11 & 96.30 & 46.65 & 0.1172 \\
%             % PointNet$^{++}$ \cite{qi2017pointnet++} + t-smooth  & 44.77 & 95.90 & 45.62 & 0.1101 \\
%             % \hline
%             % Ours (bidirectional) & 35.72 & 85.79 & 31.92 & 0.0937 \\
%             % Ours (bidirectional 1024) & 48.97 & 95.00 & 42.32 & 0.1269 \\
%             I3D & 65.56 & 92.99 & 56.04 &  0.6670 \\
%             PointNet$^{++}$ \cite{qi2017pointnet++} 1 & 71.05 & 93.53 & 45.95 &  0.1077 \\
%             \hline
%             Ours &  &  &  &  \\
%          \bottomrule
%     \end{tabular}
%     \caption{IKEA Ego 3D results for the \textit{top10} setting. }
%     \label{tab:results:baseline:ikeaego_top10}
% \end{table}

